Metabolic Regulatory Network Kinetic Modeling with Multiple Isotopic Tracers for iPSCs

The rapidly expanding market for regenerative medicines and cell therapies highlights the need to advance the understanding of cellular metabolisms and improve the prediction of cultivation production process for human induced pluripotent stem cells (iPSCs). In this paper, a metabolic kinetic model was developed to characterize underlying mechanisms of iPSC culture process, which can predict cell response to environmental perturbation and support process control. This model focuses on the central carbon metabolic network, including glycolysis, pentose phosphate pathway (PPP), tricarboxylic acid (TCA) cycle, and amino acid metabolism, which plays a crucial role to support iPSC proliferation. Heterogeneous measures of extracellular metabolites and multiple isotopic tracers collected under multiple conditions were used to learn metabolic regulatory mechanisms. Systematic cross-validation confirmed the model's performance in terms of providing reliable predictions on cellular metabolism and culture process dynamics under various culture conditions. Thus, the developed mechanistic kinetic model can support process control strategies to strategically select optimal cell culture conditions at different times, ensure cell product functionality, and facilitate large-scale manufacturing of regenerative medicines and cell therapies.

==> latexmacro.tex <==

%% LaTeX2e file `latexmacro.tex'
%% generated by the `filecontents' environment
%% from source `Gkmn51' on 2001/03/06.
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  This macro contains definitions of new \LaTeX commands  %%
%%  that are frequently used by Barry L. Nelson.  This is   %%
%%  a new release of the 'latexmacro.tex' file that I have  %%
%%  distributed for some time.  This release                %%
%%  is designed to be compatible with previous releases,    %%
%%  except for eliminating the \smallheads command.         %%
%%                                                          %%
%%  This releases fixes a few bugs (please report any you   %%
%%  find to nelsonb@random.eng.ohio-state.edu), includes    %%
%%  more documentation, and completes the definitions of    %%
%%  bold-face mathematics characters.                       %%
%%                                                          %%
%%  release 2.01   1/2/92                                   %%
%%  unreleased update 6/9/92  6/22/92 1/19/93 2/3/93        %%
%%                    6/2/93  8/15/93 11/11/93 11/23/93     %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% USING THE MACRO:
%% If you name this file latexmacro.tex, then use the following
%% statement just after the \documentstyle{} command:
%%
%%    \input [path] latexmacro
%%
%% LINE SPACING:
%% Define single, one and a half, and double space commands; these
%% may be used anywhere after \begin{document}
%%
\def\double{\par\baselineskip=24pt}
\def\single{\par\baselineskip=12pt}
\def\oneandahalf{\par\baselineskip=18pt}
%%
%% TEXT DIMENSIONS
%% Define text widths \standard, \proceedings and \myletter.
%% \proceedings prints a single, narrow column near the edge of the page.
%% Use these before \begin{document} command.
%%
\def\standard{\oddsidemargin=0in
              \evensidemargin=0in
              \topmargin =-.5in
              \textheight=8.5in
              \textwidth=6.5in}
\def\proceedings{\oddsidemargin=-.5in
                 \evensidemargin=-.5in
                 \textwidth=4.56in
                 \parindent=0.3in
                 \topmargin=-1in
                 \textheight=10in
                 \pagestyle{empty}}
\def\myletter{\oddsidemargin=.3in
                 \evensidemargin=.3in
                 \baselineskip=16pt
                 \textwidth=5.5in
                 \pagestyle{empty}}
%%
%% Define command to pull in letterhead file.
%% This command is specific to VAX/VMS and Arbortext dvips program.
%% Insert your own path.
%%
\def\letterhead{\special{ps: plotfile [is.nelson.com]letterhead.tex 
local}}
%%
%%
%% LISTS:
%% Define \plainlist environment
%%
\newenvironment{plainlist}
{\begin{list}%
{}{\setlength{\leftmargin}{\rightmargin}\setlength{\labelwidth}{0in}}}%
{\end{list}}
%%
%% Define \hangref environment for hanging indentation
%%
\newenvironment{hangref}{\begin{list}{}{\setlength{\itemsep}{0pt}%
\setlength{\parsep}{0pt}\setlength{\leftmargin}{+\parindent}%
\setlength{\itemindent}{-\parindent}}}{\end{list}}
%%
%%
%%
%%
%% MATHEMATICS:
%%Special math symbols
%%
%% operators
\def\E{{\rm E}}
\def\Var{{\rm Var}}
\def\Cov{{\rm Cov}}
\def\Corr{{\rm Corr}}
\def\Bias{{\rm Bias}}
\def\MSE{{\rm MSE}}
\def\CP{{\rm CP}}
\def\trace{{\rm trace}}
\def\tr{{\rm tr}}
%%
%% bold face roman
\def\bA{{\bf A}}
\def\ba{{\bf a}}
\def\bB{{\bf B}}
\def\bb{{\bf b}}
\def\bC{{\bf C}}
\def\bc{{\bf c}}
\def\bD{{\bf D}}
\def\bd{{\bf d}}
\def\bE{{\bf E}}
\def\be{{\bf e}}
\def\bF{{\bf F}}
\def\boldf{{\bf f}}
\def\bG{{\bf G}}
\def\bg{{\bf g}}
\def\bH{{\bf H}}
\def\bh{{\bf h}}
\def\bi{{\bf i}}
\def\bI{{\bf I}}
\def\bJ{{\bf J}}
\def\bj{{\bf j}}
\def\bK{{\bf K}}
\def\bk{{\bf k}}
\def\bL{{\bf L}}
\def\bl{{\bf l}}
\def\bM{{\bf M}}
\def\bm{{\bf m}}
\def\bN{{\bf N}}
\def\bn{{\bf n}}
\def\bO{{\bf O}}
\def\bo{{\bf o}}
\def\bP{{\bf P}}
\def\bp{{\bf p}}
\def\bQ{{\bf Q}}
\def\bq{{\bf q}}
\def\bR{{\bf R}}
\def\br{{\bf r}}
\def\bS{{\bf S}}
\def\bs{{\bf s}}
\def\bT{{\bf T}}
\def\bt{{\bf t}}
\def\bU{{\bf U}}
\def\bu{{\bf u}}
\def\bV{{\bf V}}
\def\bv{{\bf v}}
\def\bW{{\bf W}}
\def\bw{{\bf w}}
\def\bX{{\bf X}}
\def\bx{{\bf x}}
\def\bY{{\bf Y}}
\def\by{{\bf y}}
\def\bZ{{\bf Z}}
\def\bz{{\bf z}}
%%
%% bold face Greek (incomplete)
\def\balpha{\mbox{\boldmath $\alpha$}}
\def\bbeta{\mbox{\boldmath $\beta$}}
\def\bepsilon{\mbox{\boldmath $\epsilon$}}
\def\bvarepsilon{\mbox{\boldmath $\varepsilon$}}
\def\bDelta{{\bf \Delta}}
\def\bdelta{\mbox{\boldmath $\delta$}}
\def\boldeta{\mbox{\boldmath $\eta$}}
\def\bGamma{{\bf \Gamma}}
\def\bgamma{\mbox{\boldmath $\gamma$}}
\def\bLambda{{\bf \Lambda}}
\def\blambda{\mbox{\boldmath $\lambda$}}
\def\bmu{\mbox{\boldmath $\mu$}}
\def\bOmega{{\bf \Omega}}
\def\bpi{\mbox{\boldmath $\pi$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bPsi{{\bf \Psi}}
\def\bpsi{\mbox{\boldmath $\psi$}}
\def\bSigma{{\bf \Sigma}}
\def\bsigma{\mbox{\boldmath $\sigma$}}
\def\bTheta{{\bf \Theta}}
\def\btheta{\mbox{\boldmath $\theta$}}
\def\bXi{{\bf \Xi}}
\def\bxi{\mbox{\boldmath $\xi$}}
%%
%% misc. Greek with hats
\def\betahat{\hat \beta}
\def\bbetahat{\hat{\mbox{\boldmath $\beta$}}}
\def\bdeltahat{\hat{\mbox{\boldmath $\delta$}}}
\def\etahat{\hat{\eta}}
\def\epsilonhat{\hat{\epsilon}}
\def\bepsilonhat{\hat{\mbox{\boldmath $\epsilon$}}}
\def\bgammahat{\hat{\mbox{\boldmath $\gamma$}}}
\def\bmuhat{\hat{\mbox{\boldmath $\mu$}}}
\def\thetahat{\hat \theta}
%%
%% caligraphy letters
\def\cA{{\cal A}}
\def\cB{{\cal B}}
\def\cC{{\cal C}}
\def\cD{{\cal D}}
\def\cE{{\cal E}}
\def\cI{{\cal I}}
\def\cM{{\cal M}}
\def\cR{{\cal R}}
\def\cS{{\cal S}}
\def\cT{{\cal T}}
\def\cY{{\cal Y}}
%%
%% tt letters
\def\tS{{\tt S}}
\def\tC{{\tt C}}
\def\tI{{\tt I}}
\def\tT{{\tt T}}
%%
%% vec notation
\def\vp{\vec{p}}
\def\bvP{\vec{{\bf P}}}
%%
%% bold face numbers
\def\b1{{\bf 1}}
\def\bzero{{\bf 0}}
%%
%% \blot gives a square at end of formulas and proofs
%% (thanks to Marc Posner)
\def\blot{\quad {$\vcenter{\vbox{\hrule height.4pt
             \hbox{\vrule width.4pt height.9ex \kern.9ex \vrule 
width.4pt}
             \hrule height.4pt}}$}}
%%
%% End of latexmacro
